Preconditioned NonSymmetric/Symmetric Discontinuous Galerkin Method for Elliptic Problem with Reconstructed Discontinuous Approximation

In this paper, we propose and analyze an efficient preconditioning method for the elliptic problem based on the reconstructed discontinuous approximation method. We reconstruct a high-order piecewise polynomial space that arbitrary order can be achieved with one degree of freedom per element. This space can be directly used with the symmetric/nonsymmetric interior penalty discontinuous Galerkin method. Compared with the standard DG method, we can enjoy the advantage on the efficiency of the approximation. Besides, we establish an norm equivalence result between the reconstructed high-order space and the piecewise constant space. This property further allows us to construct an optimal preconditioner from the piecewise constant space. The upper bound of the condition number to the preconditioned symmetric/nonsymmetric system is shown to be independent of the mesh size. Numerical experiments are provided to demonstrate the validity of the theory and the efficiency of the proposed method.

==> preconditioner.tex <==
% vim:spell:tw=120:fo+=Mn:cc=120
\section{Construction and Analysis of the Preconditioner}
\label{sec_preconditioner}
%In this section, we will develop our preconditioner for the RDA method, By the definition of the reconstruction 
%operator $\mc{R}^m$, it is clearly that $\mc{R}^m$ is a linear isomorphism from $U_h^0$ to $U_h^m$. 
%Now we define a projection operator $T_0$ from $U_h^m$ to $U_h^0$
%\begin{equation}
  %a_h(T^0 u_h, v^0) := a_h(u_h, \mc{R}^m v^0), \quad \forall v^0 \in U_h^0, \,\, u_h \in U_h^m,
  %\label{eq_T0}
%\end{equation}
%and let $T: U_h^0 \rightarrow U_h^0$ be defined as $T := \mc{R}^m U_h^0$. Then the problem \eqref{eq_origin_system} can 
%be replaced by the preconditioned system
%\begin{equation}
  %T u_h = q,
  %\label{eq_preconditioned_system}
%\end{equation}
%where $q \in U_h^0$ is determined by the solution of $a_h(q, v^0) = f_h(\mc{R}^m v^0)$.

%Under the basis $\{e_i \}_{i=1}^{Ne}$ and $\{ \lambda_i \}_{i=1}^{Ne}$, we have the stiff matrix $\bm{A}^m := 
%(a_h(\lambda_i, \lambda_j))_{Ne \times Ne}$ and $\bm{A}^0 := (a_h(e_i, e_j))_{Ne \times Ne}$. Note that $\lambda_i =
%\mc{R}^m e_i$, the matrix representation of $\mc{R}^m$ is exactly the identity matrix. Then we obtain the matrix
%notations of the problems \eqref{eq_origin_system} and \eqref{eq_preconditioned_system} are
%\begin{displaymath}
  %\bm{A}^m \bm{u} = \bm{f},
%\end{displaymath}
%and 
%\begin{displaymath}
  %(\bm{A}^0)^{-1} \bm{A}^m \bm{u} = (\bm{A}^0)^{-1} \bm{f},
%\end{displaymath}
%respectively. Next, we shall detect whether the system \eqref{eq_preconditioned_system} is well conditioned. In other
%words, we want to prove that the condition number of the operator $T$, or equivalently, the matrix $(\bm{A}^0)^{-1}
%\bm{A}^m$, is independent of the mesh size $h$. Since $a_h(\cdot, \cdot)$ is symmetric, continuous and coercive, it can
%induce a norm $\anorm{u} := \sqrt{a_h(u, u)}$. 
%\begin{lemma}
  %The operator $T$ is self-adjoint with respect to $a_h(\cdot,\cdot)$.
  %\begin{displaymath}
    %a_h(T u, v) = a_h(u, T v).
  %\end{displaymath}
  %\label{le_self_adjoint}
%\end{lemma}
%\begin{proof}
  %By the definition of the operators $T$ and $T_0$, we have
  %\begin{displaymath}
  %\begin{aligned}
    %a_h(T u, v) &= a_h(\mc{R}^m T^0 u, v) \\
    %&= a_h(v, \mc{R}^m T^0 u) \\
    %&= a_h(T^0 v, T^0 u) \\
    %&= a_h(T^0 u, T^0 v) \\
    %&= a_h(u, \mc{R}^m T^0 v) \\
    %&= a_h(u, Tv)
  %\end{aligned}
  %\end{displaymath}
%\end{proof}
%With the help of this property, we may define the condition number of the operator $T$ under the norm $\anorm{\cdot}$ as
%\begin{equation}
  %\kappa(T) := \frac{\lambda_{\max}^a(T)}{\lambda_{\min}^a(T)},
  %\label{eq_definition_of_condition_number}
%\end{equation}
%where $\lambda_{\max}^a(T)$ and $\lambda_{\min}^a(T)$ are extreme eigenvalues of $T$ under the norm $\anorm{\cdot}$, 
%which can be represented by the Rayleigh quotation
%\begin{displaymath}
  %\lambda_{\min}(T) = \min_{u \neq 0, \ u \in U_h^0} \frac{a_h(Tu, u)}{a_h(u,u)}, \qquad \lambda_{\max}(T) = 
  %\max_{u \neq 0, \ u \in U_h^0} \frac{a_h(Tu, u)}{a_h(u,u)}.
%\end{displaymath}

%To get the estimation of the $\kappa(T)$, the following two lemmas are crucial.
%\begin{lemma}
  %For all $u^0 \in U_h^0$, there exists a constant $C_0$ independent of the mesh size $h$ such that
  %\begin{equation}
    %a_h(u^0, u^0) \leq C_0 a_h(\mc{R}^m u^0, \mc{R}^m u^0).
    %\label{eq_min_eig}
  %\end{equation}
  %\label{le_min_eig}
%\end{lemma}
%\begin{proof} 
  %It is sufficient to verify the following inequality 
  %\begin{displaymath}
    %\enorm{u^0}^2 \leq C \enorm{\mc{R}^m u^0}^2,
  %\end{displaymath}
  %which is
  %\begin{displaymath}
    %\sum_{e \in \MEh} h_e^{-1} \| \jump{u^0} \|^2_{L^2(e)} \leq C(\sum_{K \in \MTh} \| \nabla \mc{R}^m u^0
    %\|^2_{L^2(K)} + \sum_{e \in \MEh} h_e^{-1} \| \jump{\mc{R}^m u^0} \|^2_{L^2(e)}),
  %\end{displaymath}
  %due to the continuity \eqref{eq_continuity} and the coercivity \eqref{eq_continuity}. For $e \in \MEh^i$, there 
  %exist $K_0, K_1 \in \MTh$ such that $e = \partial K_0 \cap \partial K_1$. Let $\bm{x}_{K_0}$ and $\bm{x}_{K_1}$ be 
  %the barycenter of $K_0$ and $K_1$, respectively. From the constraint in \eqref{eq_leastSquares}, we have
  %\begin{displaymath}
    %u^0(\bm{x}_{K_0}) = (\mc{R}^m u^0)(\bm{x}_{K_0}), \quad u^0(\bm{x}_{K_1}) = (\mc{R}^m u^0)(\bm{x}_{K_1}).
  %\end{displaymath}
  %We denote by $\bm{p}_e$ a point on $e$. Applying the inverse inequality \eqref{eq_inverse}, we get
  %\begin{displaymath}
    %\begin{aligned}
    %h_e^{-1} \| \jump{u^0} \|_{L^2(e)}^2 &= h_e^{-1} \| (\mc{R}^m u^0)(\bm{x}_{K_0}) 
    %- (\mc{R}^m u^0)(\bm{x}_{K_1}) \|_{L^2(e)}^2
    %\\
    %& \leq C h^{d-2} | (\mc{R}^m u^0)(\bm{x}_{K_0}) - (\mc{R}^m u^0)(\bm{x}_{K_1}) |^2 \\
    %& \leq C h^{d-2} (| \ (\mc{R}^m u^0)(\bm{x}_{K_0}) - (\mc{R}^m u^0)(\bm{p}_e) |_{K_0} \ |^2 + |\ (\mc{R}^m u^0)
    %(\bm{p}_e)|_{K_0} - (\mc{R}^m u^0)(\bm{p}_e) |_{K_1} \ |^2 \\
    %& \qquad \qquad + | \ (\mc{R}^m u^0)(\bm{p}_e) |_{K_1} - (\mc{R}^m u^0)(\bm{x}_{K_1}) \ |^2 ) \\
    %& \leq C h^{d-2} (h^2 \| \nabla (\mc{R}^m u^0) \|_{L^\infty(K_0 \cup K_1)}^2 + \| \jump{\mc{R}^m u^0} \|_{L^\infty(e)}^2 ) \\
    %& \leq C \| \nabla (\mc{R}^m u^0) \|_{L^2(K_0 \cup K_1)}^2 + C h^{-1} \| \jump{\mc{R}^m u^0} \|_{L^2(e)}^2
    %\end{aligned}
  %\end{displaymath}
 %Similarly, for $e \in \MEh^b$, suppose $e \subset \partial K$. Let $\bm{x}_{K}$ be the barycenter of $K$, we obtain
 %\begin{displaymath}
   %\begin{aligned}
     %h_e^{-1} \| \jump{u^0} \|_{L^2(e)}^2 &= h_e^{-1} \| u^0 \|^2_{L^2(e)} \\ 
     %&\leq C h^{d-2} |(\mc{R}^m u^0)(\bm{x}_{K}) |^2 \\
     %&\leq C h^{d-2} (|(\mc{R}^m u^0)(\bm{x}_{K}) - (\mc{R}^m u^0)(\bm{p}_e)|^2 + |(\mc{R}^m u^0)(\bm{p}_e) |^2) \\
     %&\leq C \| \nabla (\mc{R}^m u^0) \|^2_{L^2(K)} + C h^{-1} \| \jump{\mc{R}^m u^0} \|_{L^2(e)}^2.
   %\end{aligned}
 %\end{displaymath}
 %Finally, \eqref{eq_min_eig} can be verified by summing the above inequalities over all $e \in \MEh$, which completes 
 %the proof. 
%\end{proof}

%\begin{lemma}
  %For all $u^0 \in U_h^0$, there exists a constant $C_1$ independent of the mesh size $h$ such that
  %\begin{equation}
    %a_h(\mc{R}^m u^0, \mc{R}^m u^0) \leq C_1 a_h(u^0, u^0).
    %\label{eq_max_eig}
  %\end{equation}
  %\label{le_max_eig}
%\end{lemma}
%\begin{proof}
  %It is sufficient to verify the following inequality 
  %\begin{displaymath}
    %\enorm{\mc{R}^m u^0}^2 \leq C \enorm{u^0}^2,
  %\end{displaymath}
  %which is
  %\begin{displaymath}
    %\sum_{K \in \MTh} \| \nabla \mc{R}^m u^0 \|^2_{L^2(K)} + \sum_{e \in \MEh} h_e^{-1} \| \jump{\mc{R}^m u^0} 
    %\|^2_{L^2(e)} \leq C \sum_{e \in \MEh} h_e^{-1} \| \jump{u^0} \|^2_{L^2(e)}.
  %\end{displaymath}
  %For any element $K \in \MTh$, we let 
  %\begin{displaymath}
    %u^0_{\max, K} := \max \{ u^0|_{K'}; K' \in S(K) \}, \quad u^0_{\min, K} := \min \{ u^0|_{K'}; K' \in S(K) \}.
  %\end{displaymath}
  %By the stability of $\mc{R}^m$ \eqref{eq_recons_stability} and the inverse inequality \eqref{eq_inverse}, we have
  %\begin{displaymath}
    %\begin{aligned}
      %\| \nabla (\mc{R}^m u^0) \|^2_{L^2(K)} &= \| \nabla (\mc{R}^m u^0 - u^0_{\min, K}) \|_{L^2(K)}^2 \\
      %&\leq C h^{d-2} \| \mc{R}^m (u^0 - u^0_{\min, K}) \|^2_{L^\infty(K)}  \\
      %&\leq C \Lambda(m, K)^2 h^{d-2} \| u^0 - u^0_{\min, K} \|_{L^\infty(S(K))}^2 \\
      %&\leq C \Lambda(m, K)^2 h^{d-2} \| u^0_{\max, K} - u^0_{\min, K} \|_{L^\infty(S(K))}^2.
    %\end{aligned}
  %\end{displaymath}
  %For any $e \in \MEh^i$, let $e = \partial K_0 \cap \partial K_1$ and $\bm{x}_{K_0}$ and $\bm{x}_{K_1}$ be 
  %the barycenter of $K_0$ and $K_1$, respectively. We denote by $p_0 = (\mc{R}^m u^0) |_{K_0}$, 
  %$p_1 = (\mc{R}^m u^0) |_{K_1}$. Using \eqref{eq_leastSquares} and the inverse inequality \eqref{eq_inverse}, we obtain
  %\begin{displaymath}
    %\begin{aligned}
      %h_e^{-1} \| \jump{\mc{R}^m u^0} \|_{L^2(e)}^2 &= h_e^{-1} \| p_0 - p_1 \|_{L^2(e)}^2 \\
    %&\leq C(h^{-1} \| p_0 - p_0(\bm{x}_{K_0}) \|^2_{L^2(e)} + h^{-1} \| p_0(\bm{x}_{K_0}) - p_1(\bm{x}_{K_1}) \|^2_{L^2(e)}
    %+ h^{-1} \| p_1(\bm{x}_{K_1}) - p_1\|^2_{L^2(e)}) \\
    %&\leq C h^{d-2} (\| p_0 - p_0(\bm{x}_{K_0}) \|^2_{L^\infty(e)} + \| p_1 - p_1(\bm{x}_{K_1}) \|^2_{L^\infty(e)} 
    %+ h^{-1} \| \jump{u^0} \|^2_{L^2(e)} )\\
    %&\leq C h^d (\| \nabla p_0 \|^2_{L^\infty(K_0)} + \| \nabla p_1 \|^2_{L^\infty(K_1)} + h^{-1} \| \jump{u^0}
    %\|^2_{L^2(e)}) \\ 
    %&\leq C (\| \nabla (\mc{R}^m u^0) \|_{L^2(K_1 \cup K_2)}^2 + h^{-1} \| \jump{u^0} \|^2_{L^2(e)}).
    %\end{aligned}
  %\end{displaymath}
  %For any $e \in \MEh^b$, $e \subset \partial K$, let $\bm{x}_K$ be the barycenter of $K$ and $p = (\mc{R}^m u^0) |_K$. 
  %Analogously, we have
  %\begin{displaymath}
    %\begin{aligned}
      %h_e^{-1} \| \jump{\mc{R}^m u^0} \|_{L^2(e)}^2 &= h_e^{-1} \| p \|_{L^2(e)}^2 \\
      %&\leq C(h^{-1} \| p - p(\bm{x}_K) \|^2_{L^2(e)} + h^{-1} \| p(\bm{x}_K) \|^2_{L^2(e)}) \\
      %&\leq C ( h^{d-2} \| p - p(\bm{x}_K) \|^2_{L^\infty(e)} + h^{-1} \| p(\bm{x}_K) \|^2_{L^2(e)}) \\
      %&\leq C (\| \nabla(\mc{R}^m u^0) \|^2_{L^2(K)} + h^{-1} \| \jump{u^0} \|^2_{L^2(e)}).
    %\end{aligned}
  %\end{displaymath}
  %It remains to bound $h^{d-2}\| u^0_{\max, K} - u^0_{\min, K} \|$ over the patch $S(K)$. Suppose the maximum and 
  %minimum of $u^0$ attain at $K_M$ and $K_m$, respectively, that is $u^0_{\max, K} = u^0|_{K_M}$, $u^0_{\min, K} = 
  %u^0|_{K_m}$. Since the element patch is a connected set, we can always find a broken line in $S(K)$ which starts at 
  %$\bm{x}_{K_M}$ and ends at $\bm{x}_{K_m}$. Suppose the elements which the broken line passes in sequence are 
  %$K_0 = K_M, K_1, \dots, K_l = K_m$, then we find
  %\begin{displaymath}
    %\begin{aligned}
      %h^{d-2} \| u^0_{\max} - u^0_{\min} \|^2 &\leq C h^{d-2} (\| u^0_{K_0} - u^0_{K_1} \|^2 + \| u^0_{K_1} - u^0_{K_2} 
      %\|^2 + \dots + \|u^0_{K_{l-1}} - u^0_{K_l} \|^2) \\
      %&\leq C \sum_{e \subset S(K)} h^{-1} \| \jump{u^0} \|_{L^2(e)}^2.
    %\end{aligned}
  %\end{displaymath}
  %The proof is completed by summing the above inequalities over all $K \in \MTh$ and $e \in \MEh$.
%\end{proof}
%Now we are ready to give an estimate to the condition number of the operator $T$.
%\begin{theorem}
  %The minimum eigenvalue of $T$ is lower bounded by $1/C_0$ and the maximum eigenvalue of $T$ is upper bounded by $C_1$,
  %so the condition number of $T$ satisfies
  %\begin{equation}
    %\kappa(T) \leq C_0C_1
    %\label{eq_estimate_KT}
  %\end{equation}
  %\label{th_estimate_KT}
%\end{theorem}
%\begin{proof}
  %By the definition of $T$ and lemma \ref{le_max_eig}, for all $u_h \in U_h^m$, we have
  %\begin{displaymath}
    %\begin{aligned}
      %a_h(Tu_h, T u_h) &= a_h(\mc{R}^m T^0 u_h, \mc{R}^m T^0 u_h) \\
      %&\leq C_1 a_h(T^0 u_h, T^0 u_h) \\
      %&= C_1 a_h(u_h, T u_h) \\
      %&\leq C_1 a_h(u_h, u_h)^{1/2} a_h(T u_h, T u_h)^{1/2}.
    %\end{aligned}
  %\end{displaymath}
  %Hence,
  %\begin{displaymath}
    %a_h(T^2 u_h ,u ) \leq C_1^2 a_h(u_h, u_h),
  %\end{displaymath}
  %which implies $\lambda_{\max}(T^2) \leq C_1^2$, so that $\lambda_{\max}(T) \leq C_1$. To get the lower bound of 
  %$\lambda_{\min}(T)$, we analyse the maximum eigenvalue of $T^{-1}$. For all $u_h \in U_h^m$, let $u^0 \in U_h^0$ such
  %that $u_h = \mc{R}^m u^0$. Then we see that
  %\begin{displaymath}
    %a_h(T^{-1} u_h, u_h) = a_h(T^{-1} u_h, \mc{R}^m u^0) = a_h(T^0 T^{-1} u_h, u^0).
  %\end{displaymath}
  %Besides, it can be shown that 
  %\begin{displaymath}
    %\mc{R}^m(T^0 T^{-1} u_h) = (\mc{R}^m T^0) (\mc{R}^m T^0)^{-1} u_h = u_h.
  %\end{displaymath}
  %Recall the fact that $\mc{R}^m$ is a linear isomorphism from $U_h^0$ to $U_h^m$, so $T^0 T^{-1} u_h = u^0$. Thus we 
  %get
  %\begin{displaymath}
    %a_h(T^{-1} u_h, u_h) = a_h(u^0, u^0),
  %\end{displaymath}
  %which means $\lambda_{\max}(T^{-1}) \leq C_0$ or equivalent, $\lambda_{\min}(T) \geq \frac{1}{C_0}$. Then we arrive 
  %at the final conclusion $\kappa(T) \leq C_0 C_1$ and complete the proof.
%\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "article"
%%% End:

